`It is currently hodgepodge'': Examining AI/ML Practitioners' Challenges during Co-production of Responsible AI Values

Recently, the AI/ML research community has indicated an urgent need to establish Responsible AI (RAI) values and practices as part of the AI/ML lifecycle. Several organizations and communities are responding to this call by sharing RAI guidelines. However, there are gaps in awareness, deliberation, and execution of such practices for multi-disciplinary ML practitioners. This work contributes to the discussion by unpacking co-production challenges faced by practitioners as they align their RAI values. We interviewed 23 individuals, across 10 organizations, tasked to ship AI/ML based products while upholding RAI norms and found that both top-down and bottom-up institutional structures create burden for different roles preventing them from upholding RAI values, a challenge that is further exacerbated when executing conflicted values. We share multiple value levers used as strategies by the practitioners to resolve their challenges. We end our paper with recommendations for inclusive and equitable RAI value-practices, creating supportive organizational structures and opportunities to further aid practitioners.

==> drafts/1.__IMP__literature-expanded.tex <==
\section{Related Work}

\subsection{What is Responsible AI?}
In the last decade, Responsible AI (RAI) has grown to encompass an expected push of making AI/ML field more accountable for its outcomes \cite{asken2019therole}. However, to date, there is a lack of consensus on the definition of RAI. Previous studies define RAI both as a noun (responsibilities of AI  \cite{abrassart_2017}) and a verb (AI being responsible \cite{Dignum_2019}. Multifaceted and interdisciplinary efforts are being made towards making the AI/ML community considerate of the diverse socio-technical impacts on society where such technologies are deployed \cite{Dignum_2021}. Scholars have used ``society'' in a broader context to illustrate that a balanced approach is needed that is inclusive of roles such as marginalized users, policymakers, ethicists, practitioners, designers, etc. \cite{Dignum_2021}. 

Some say that the roots of RAI can be found in the foundational studies in Ethical AI that brings a critical lens to the AI field  \cite{khan1995,Gips1994, ashurst2022} (often overlapping with machine Ethics \cite{Robbins2019}). Consequently, studies within Ethical AI have contributed to RAI in diverse ways. A strand of research consists of meta-studies, focusing on the core ethical AI concepts to provide nuances and richness to the AI conversations \cite{Harris_Anthis_2021a}. Another strand of studies have focused on empirical analysis of critical ethical problems (e.g., trolly problems) \cite{peter2019, yu2018, Mittelstadt_2019, Awad_2018} and operationalizing broad ethical principles and values into concrete AI/ML scenarios and stages (e.g., virtue ethics) \cite{Gips1994,hooker2018}. These studies have also led to several studies recommending comprehensive ethical guidelines within the contexts of AI/ML. \cite{Vakkuri_Abrahamsson_2018,Harris_Anthis_2021a, ethical2019, Hagendorff_2020, Jobin_Ienca_Vayena_2019}. 


RAI studies have also drawn their inspiration from research on AI for Social Good (or AI4SG) \cite{ryan2020}. Research in AI4SG has focused on implementing AI/ML systems with an aim to create positive impact in the community \cite{Berendt_2019}. Studies within the field have further discussed that eliciting values (e.g., solidarity \cite{Floridi_2018}) and methods (e.g., capabilities approach \cite{bondi2021}) can be closely aligned to the Sustainable Development Goals of UN \cite{Ghallab_2019} mentioned in the previous section. AI4SG has been applied and critically studied across multiple fields, such as agriculture \cite{madaan2019}, health \cite{Azra2021}, and education \cite{cannanure2020} to illustrate the broad range of impact by Responsible AI related decision-making. AI4SG has also helped community understand the impact of AI systems on the ground, especially on underserved and marginalized communities in Global North and Global South \cite{chinasa2021, wang2021}. For example, \citet{sambasivan2022} studied dataworkers who collect data for ML models to show how their work is often de-valued within the overall. 

%At the same time the vagueness associated with 
``Ethical'' and ``Social good'' \cite{moore2019ai, green2019good} research communities have significantly focused on a subset of values. Two such values were accountability and trustworthiness of AI systems  that contributed to the need for a more nascent movement of \textit{explainable AI} \cite{doran2017, Barredo_2020}. Subsequently, more scholars have since recognized that explainability needs vary across groups of individuals with and without a background in AI (i.e., ML practitioners and end-users) \cite{ehsan2021}. These different individuals also require different approaches in making AI systems accountable. A similar movement within purview of RAI focused on specific values of FATE (Fairness, Accountability, Transparency, and Ethics/Explainability) \cite{Shin_Park_2019, Licht_2020, kroll165accountable}. For instance, \citet{Mitchell_2021} in their study bring out disparities in the notion of fairness that is used while making prediction-based decision making, calling out the trade-off practices that are employed in the field.

As is evident, RAI has emerged as an umbrella term that encapsulates the aforementioned movements through collective actions and responsibilities that are equally shared by different stakeholders involved in ML/AI \cite{Askell2019}. Moreover, values underlying RAI movements have played a key role in encouraging interdisciplinary conversations across multiple roles in the pursuit of RAI. In the next section, we unpack the notion of some of these values, examine their roots in HCI, and their present role in RAI. 

\subsection{Collective Values in Responsible AI: HCI perspectives}
The field of Technology studies have been long fascinated with values as an aspect of overall social \cite{mackenzie1999social} and political \cite{winner1986artifacts, Star_1999} contexts and how they are embedded in technology systems \cite{latour1992missing}. Studies within HCI have built on this foundation of value examination to develop directed outcomes specific to the context of technology, design, development, and longitudinal usage. Initial set of studies by Nissanbaum and colleagues have explored how values are embodied in the technology through deliberate design practices \cite{flanagan2008embodying, friedman97}, arguing against the previously held belief that technology is often ``value-neutral''. These criticisms paved the way for researchers to bring ethical, socio-technical, and political concerns into technology development.

\textit{Value-sensitive Design} (VSD) by \citet{Friedman2013} is a step in this direction. Over the years, it has matured into a holistic framework that enables technology creators to not only use values to reflect technological affordances (conceptual and empirical enquiry) but also use them as action lens to architect technological solutions (technological enquiry) \cite{Friedman2021, Hendry2021}. Over the years, VSD has been extended in several ways, often in response to its criticisms. \citet{dantec2009} built upon the theoretical and epistemological perspectives of VSD by developing empirical methods to illicit value discovery and reflection.
\citet{Jafari2015a} took a more critical perspective by making a distinction in two ways to look at values in VSD, arguing that both studying value as \textit{noun} (or what  \citet{morris1956varieties} calls values in principle)) to identify different values in the socio-technical system and value as \textit{verb} (i.e. valuing) to understand the socio-technical process that contribute to embedded values in technological artifacts. Lastly, a significant shortcoming for VSD was its ease of applicability in industry contexts \cite{Shilton_2013}. VSD is often perceived to be a relatively slow, necessary, often requiring specialists for implementation. To overcome these challenges, Shilton introduced the use of \textit{`value levers'}, a low-cost entry point for value-oriented conversations while building technology artifacts while having value advocates in the organization \cite{shilton2018, Shilton_2013}. Regardless, aforementioned value-based theories have enabled HCI research to critically engage with value systems in different contexts, such as 
work \cite{wong2021}, education \cite{Aleven_2019}, health \cite{barry2017}, especially focusing on marginalized communities \cite{houston2016}. Researchers have further argued that just creating a list of values is not sufficient in technology design and significant research is needed to enable practitioners to collaboratively create values socially \cite{borning2012next}.

% \bheading{Transition of values into ML/AI}
More recently, they have started playing a key role in shaping the increased emphasis on studying and shaping values within ML/AI. However, the initial focus on values was primarily on computational in nature, such as performance \cite{}, generalizability \cite{}, and efficiency \cite{} that received primary attention \citet{birhane2022}. It is only very recently with the \textit{responsible AI} and similar movements that the focus is shifting from values around computational issues to values around societal and ethical issues \cite{birhane2022}. In the following few paragraphs we explore how values have taken a mature shape in the emerging sub-field of responsible AI/ML. Early scholarship in responsible AI/ML have emphasized on inherent issues and biases in the models by studying absence of important ethical values when applied to complex, real world situations. \citet{burrell2016} explored one such issue: lack of transparency in ML models, contributing to sociopolitical issues at different levels. For instance, she demonstrates how complex ML models have inherent interpretability issues  stemming from lack of transparency on how predictions were achieved. Several other studies have taken a similar approach and explored individual values that they felt were critical for the models to reflect towards the society. Some of these values included fairness \cite{}, explainability \cite{doran2017}, and non-malfeasance or non-harm \cite{Jobin_Ienca_Vayena_2019}. A common underlying assumption among these studies were that values were enacted in their own spaces. Only recently, there is a shift in this outlook by a few studies that have adopted \citet{Friedman's} perspective that values do not exist in isolation, often occupying overlapping and contested spaces \citet{yurrita2022}. Our study aims to provide deeper insights within this complex space of multiple values.  

Another dimension that has been explored is whose targeted values are important  \cite{borning2012next} and should be considered while producing AI/ML algorithms.End-users values have been an important consideration for several studies, lending a critical lens around the current models deployed in the wild. This has helped scholars understand value impact and implications on the end-users at community and societal level \cite{kizilcec2020, Wong_2020, smith2020, robertson2020}. These studies contested the idea that development of fair algorithms is primarily conceptualized as a technical task without taking end-users' values into consideration \cite{Haubermann_Lutge_2022}. For example, \citet{robertson2021} investigated educational ecosystem where ML models were deployed to map students to schools to show how algorithmic values and parents values were constantly at odds with each other. These studies also laid foundation to action-research around values (e.g. participatory approaches \cite{delgado2021}) to design toolkits, frameworks, and guidelines that accommodate end-user values in producing ML models \cite{Katell2020, krafft2021, shen2022The}.

A parallel set of studies have also recognized the importance of understanding different practitioners' values who are tasked with producing responsible algorithms,  such as data scientists \cite{passi2019problem}, designers \cite{Yildirim2022How}, scientists, and engineers \cite{Sheuerman2020how} among others. More recently, researchers have drawn attention to values of lesser explored roles, whose work is often invisible, but contribute to the critical human infrastructure responsible for collecting data on the ground \citet{thakkar2022}. Such practitioner-focused studies are critical in understanding ``how'' and ``why'' particular values are embedded in AI/ML models early on in the life-cycle. However, majority of the studies have explored the values of particular practitioners in silos, often in exclusion with other practitioner roles in the life-cycle. 

Recently, scholars have begun to explore practitioners' collective values. For example \citet{madaio2020codesign} focused on controlled settings, where specific practitioners' values  could co-design fairness checklist as one of their RAI Values. \citet{jakesh2022how} explored a more broader set of values of practitioners and compared it against that of end-users in an experimental setting. Another relevant study by \citet{rakova2021} has explored RAI decision-making in an organizational setting without explicitly invoking values, laying a roadmap to get from current state to aspirational RAI practices. Our study adds to this relevant literature in a few ways. First, our study goes beyond the scenario-based/controlled settings/experimental setups by focusing on natural work settings and co-production in those settings. Second, we focus on co-production among diversity of stakeholder roles who are making an explicit effort to recognize and incorporate RAI values, unlike silo-ed studies previously. Third, our study extends \cite{rakova2021} by explicitly unpacking the co-production challenges that are deeply rooted in RAI values. To this end, we answer the following research questions:\\ \textbf{(RQ 1): \textit{What are the current industry challenges in enabling RAI value co-production among diverse AI/ML practitioners?}\\ }
\textbf{(RQ 2): \textit{How do diverse AI/ML practitioners overcome challenges as they align their RAI Values ?}}\\

% \textbf{RQ-1:} \textit{What are the current industry structures that enable enable RAI value conversations among AI/ML practitioners?} \\ 
% \textbf{RQ-2:} \textit{How do AI/ML practitioner utilize the structures to co-produce RAI values?}
\subsection{Employing Co-production}
To answer our research questions, we employed the conceptual framework of \textit{co-production} proposed by \citet{jasanoff2004idiom}. Co-production was originally developed by Elinor Ostrom to emphasize the integral role users played in producing public goods \cite{ostrom:2009}. She defined co-production as the activities where state actors and the individuals of the community come together to create effective and useful services \cite{ostrom1999crossing}. Over the years, this notion has been developed further in different academic disciplines, including HCI \cite{carroll2016} and Science Technology \& Studies \cite{jasanoff2004idiom}, producing heterogeneous definitions.

Within HCI, researchers have adopted the definition of co-production from studies that explored the practices of professionals and its impact on social exchanges between professionals and citizens in domains like health \citet{Eijk_Steen_2014} and education \citet{porter2013co}. For instance, \citet{keegan2016} explored the co-production practices between editors in producing knowledge to the publics. Other examples include recent work in community informatics \cite{Chen_2019,Chen2_2019, cahn2013co}. Within these studies, the role of technology has been largely viewed as an enabler for co-production. It is seldom that the role of technology designers and technology institutions have been studied as active co-producers alongside other practitioners. Research in STS has taken a more critical approach by bringing accountability on technology designers within co-production to the forefront \cite{}. In particular, \citet{jasanoff2004idiom} defined co-production more broadly to include deliberations undertaken by non-state actors like technology corporations and research organizations that have huge impact on the communities that they are serving. Jasanoff embraced an \textit{international lens} on co-production, arguing that understanding these co-production activities offered new ways to understand the impact of new technological practices, expertise, knowledge, and material objects in the society they are produced to serve. It also helps visualizing relationship between knowledge and practice. At core, Jasanoff's co-production framework not only places importance on how establishments organize or express themselves, but also about what they value and how they assume responsibility for their inventions.

To explore these different facets, Jasanoff proposed four sites of co-production that are worth investigating. First site of exploration are \textit{identities}: roles and relationships of different actors that form the foundation for co-production activities. Second site of exploration are the \textit{institutions} containing different structures that empower or hinder individuals to co-produce. Third site is examining different type of \textit{discourse} that occur as part of the co-production activities. Solving technological problems often involves discourses producing new knowledge and linking such knowledge to practice. Last site of co-production is \textit{representations} produced both during co-production to facilitate discourses as well as after co-production in the form of end-product. Overall, the four sites of co-production framework proposed by Jasanoff are appropriate to understand the initiatives around RAI values for multiple reasons. First, technological corporations developing AI/ML innovations have strong bi-directional relationship with their communities, and within these organizations. Second, for successful RAI value implementation, practitioners need to leverage the complex structures within their organizations that are invisible to external communities. Third, RAI value implementations occur through strategic discourses and deliberations that translate knowledge to effective execution. Fourth, in the process of RAI value deliberations, individuals co-create representations that further the implementation efforts of RAI.













==> drafts/5-1institutions.tex <==
\section{Findings}

\blue{Our overall findings are divided into three sections. The first section introduces the \textit{institutional structures} that facilitated RAI values co-production among practitioners. %We call it \textit{value elicitation}, a process by which practitioners externalize their RAI values and associated perceptions with the peers. 
The second section dives deeper into these structures by exploring how AI/ML practitioners participate in \textit{discourses} through prioritization and deliberation of RAI values within their teams. We also present major tensions, that arise in the discourses. 
The third section lists different alignment strategies used to generate consensus on RAI values. Through out these sections, we explore different value levers \cite{Shilton_2013}, carefully thought out activities that enable different forms of value negotiations and engagement, developed and used by different practitioners and institutions to promote co-production of values.}
 
\subsection{Institutional Structures for RAI Value Co-production}

\blue{Institutional structures are essential in enabling co-production of new knowledge \cite{Jasanoff_2004}. It is these structures that facilitate relationships for deliberation, standardize democratic methods, validate safety of new technological systems, before information is disseminated into the society. We found two key institutional structures that enabled deliberation around RAI values within AI/ML companies.}

% These structures were leveraged by roles that focused on end-products and there fore motivated by the experiences of the end-users. Consequently, the RAI values they shared and deliberated were very broad and diverse. Example values included \fixme{Explainability (end-user), privacy, non-maleficence, trust and safety, diversity, equity, social justice, agency, and community innovation, among others. Second were top-down structures that employed by the roles that were closer to design and development of ML models relied on academic insights, engineering breakthroughs, and experiences to share their RAI values. Typical RAI values \fixme{included fairness, transparency, accountability, and interpretability (along with explainability). We look at these two structures in-depth.}}
\begin{figure*}
\centering
\includegraphics[width=\linewidth]{images/VLV.png}
\caption{Value levers listed against values }
\label{fig-1}
\end{figure*}

\bheading{Bottom-up Motivated Self-vigilantes}
First type of structures were bottom-up. Within these structures RAI conversations developed through RAI value sharing in the lower echelons of organizations, often within AI/ML practitioners' own teams. In our interviews, \fixme{eight practitioners from four different organizations} experienced or initiated bottom-up practices that engaged with RAI values. One of the enablers for such bottom-up innovation was individuals' sense of responsibility towards producing AI/ML models that did not lead to any harm in society. This social responsibility was direct culmination of their backgrounds and day to day experiences in personal and work settings. For instance, \fixme{P22, a user experience researcher working in a social media company around generative models}, shared how their first hand experience of end-users on the ground formed their opinion about which RAI values to bring into the conversations with the team. 

Similarly, a few other practitioners paid close attention to `\textit{social climate}' (e.g., LGBTQ month, hate speech incidents) to elicit particular RAI values. Such individuals encouraged and convinced their teams to engage with RAI values early on in AI/ML lifecycle in order to minimize the potential harm of their ML models or AI products. They mobilized their teams to seek out RAI programs available within and outside their organization. On occasion, when such RAI programs were not available, individuals created opportunities to engage with other members within the organization. For instance, \fixme{P08}, a program manager in a large-scale technology company, shared how they developed a semi-structured workshop to encourage and support team members to come together and share RAI values. The workshops provided a safe space for individuals to find commonly grounded definitions, contextualize RAI values to their products, and prioritize those values to implement in their projects. P08 described:

\begin{quote}
    ``\textit{The initiative started with keen interest in socially responsible [AI] research and ultimately products. But we cater to projects that are very self-determined, very bottom-up that aligned with our values and priorities within the organization \dots These are what I call responsible innovation vigilantes around the company. I have also started that way but have grown into something more than that. You'll see this at the product level or at the research team level, where somebody will speak up and say, `Hey, I want to be responsible for these RAI values and make this my job and find solutions'. So you start to see individuals in different pockets of the company popping up to do RAI stuff.}''
\end{quote}

Successful bottom-up RAI programs that facilitated value elicitation covered a broad range of RAI values that were often co-determined. These programs focused on education and capacity building of teams, enabling them to define and contextualize their values. \textit{`RAI vigilantes'} also utilized several value levers in these programs.

The most commonly used levers included scenario-based narratives and adversarial role plays, open-ended and abstract activities that engaged practitioners in opinion formation and sharing. Other value levers included conducting a literature review of specific RAI values and understanding cutting-edge methods, definitions, and guidelines around them. To bring-in complementary RAI values into the team, several practitioners also deployed educational value levers. \fixme{P18}, a data scientist working in a startup, hosted a panel to capture complementary perspectives around AI explainability. Visibility into how explainability was perceived differently by different community members, such as NGOs and government, contributed to a better understanding of how to develop explainable models. In a similar example, \fixme{P09}, an engineer working on a reinforcement learning model in the context of healthcare for low resources in India, facilitated field visits to the end-user communities. The exposure helped practitioners better articulate RAI values that mattered to the end-users in the community. 

\bheading{Bottom-up Motivated Curiosity}

Apart from self-motivated social responsibility, practitioners elicited values because of their curiosity about RAI within their peer networks. This included formative questions, usually seen early in the stages of ML development. For instance, \fixme{P11}, a senior director at a health technology company who oversaw RAI initiatives, shared that several practitioners reached out to discuss what ``\textit{fairness}'' as an RAI value should mean to them and their teams. The common questions included ones about operationalizing RAI using ML, such as, ``\textit{How does fairness apply to rule-based models? What kind of RAI values to invoke while collecting data?’’} and ones about operationalizing RAI using human-in-loop, such as, ``\textit{How should fairness apply when the decision is made by a human? How do RAI values apply differently?}’’ Usually, such curiosity was welcomed and responded to with significant educational efforts. For example, P05, a technical manager leading his team on data collection for the development of knowledge graphs, revealed how privacy was defined and materialized differently amongst collaborating partners responsible for data collection and labeling.

P05 engaged in multiple iterations of RAI value sharing and deliberation with the partners to ensure that they understood and strived towards similar RAI standards and appreciated data-hygiene practices (e.g., data cleaning and de-identification). Alternatively, values were also discovered and elicited later in the stages of ML development. In our findings, one form of reaction came in the form of academic criticism or critique around particular values that were seen concerning a particular product (e.g., ``\textit{what steps are you taking to ensure there is no bias?’’}. Another form of reaction came from end-users' behavior who experienced the models through a particular product. P20, a user experience researcher working with deep learning models in finance, shared how user feedback affected their value elicitation:

\begin{quote}
    ``\textit{Once the users use our product and we see the feedback, it makes us realize, `oh, people are sometimes using this feature in an unintended way that might in turn impact the way we are going about certain values, say transparency' \dots. Initially we were like, `We should strive for transparency by adding a lot of explanations around how our model gave a particular output'. But after a point we realized too many explanations [for transparency] fostered inappropriate trust over the feature \dots We could not have know this just through our discussions \dots It's a slow process, but gives a new understanding.}
\end{quote}
Earlier curiosity or later realization through feedback and visibility into the outcomes, both happened in a bottom-up fashion where a particular practitioner recognized the need to define and elicit values without a hierarchical top-down mandate. %In next section, we will briefly share how top-down approaches elicit values differently.  

\bheading{Implicitly \& Explicitly motivated Top-down Approaches}


While the previous section focused primarily on implicitly-motivated individuals, we discovered that such implicit motivations might also exist at an organizational level. Some opportunities for RAI value elicitation were facilitated by structures that were recognized, established, and integrated into the standardized workflows of the practitioners' teams to a varying degree. Organizations leveraged these structures to establish checkpoints and push practitioners to think and engage with RAI values around their products at an individual and team levels. We found a total of \fixme{12} individuals from 5 companies who either implemented or facilitated RAI practices at a top-down level. 

For example, \fixme{P10}, a manager who facilitated one such top-down RAI program in a large-scale technology company for AI/ML teams, described different ways in which teams engaged with him on RAI values: 

\begin{quote}
``\textit{We have a bunch of internal Web pages that point you in all different types of directions. We don't have a singular voice that the individuals can speak with \dots. Its currently hodgepodge. Some teams come to us willingly. They had already thought about some harms that could occur. They say, `Here's our list of harms, here’s some ideas on what we want to do’ They'd already done pre-work and are looking for some feedback. Other times come to us because they've been told to \dots They haven’t thought much about RAI and need longer conversations \dots Other times were are told to go track down a participant individual or team because they are doing ML stuff that will require RAI assistance, but they don't know about us}’’
\end{quote}

Alternative to P10’s narrative, we found that potential public-facing legal and ethical failures also hastened the development of RAI structures in the organizations. Objective of such RAI structures were to anticipate and reduce the likelihood of potential harms caused by the newer, complex deep learning models (e.g., transformer networks). We found several instances where particular member(s) of the team acted as a team liaison to create formal structures. Such structures usually resembled RAI programs that would kick-start several activities, such as RAI education and implementation. P19, a policy director at an RAI consultation firm, described how RAI structures that enable individuals to share their values and seek out assistance are being encouraged by the companies in response to upcoming laws, allowing them to be more compliant: 

\begin{quote}
    ``\textit{Even if you're are conservative, the current climate is such that it's going to be a year or two max from now, where you will start to have an established, robust regulatory regime for these (RAI) issues. So a good way to to get it to create the [RAI]programs in whatever capacity, that enables companies to comply with the new regulations \dots even if you have companies doing Responsible AI programs from scratch, it eventually compliance that gets them executive buy-in. }''
\end{quote}



%%\bheading {Challenges in Value Elicitation}
%%As shown in the previously, value elicitation is not a solo practice - individuals do elicit values from peer-networks, and collaborators. However, as such a practice requires working with individuals and organization structures, one has to be prepared for multiple challenges.

%%\begin{description}
%% challenge-1: Superficial
%%   \item[Education and Knowledge Gap] One of the the key issues we discovered was practitioners' difficulties to engage with RAI values beyond in depth. \fixme{P07} a policy advisor in a large technology company who regularly interacted with those who implemented RAI described it as a "superficial engagement" `\textit{moralizing}', wherein practitioners frequently struggled to develop deeper interpretations of the elicited values and contextualize them in relation to the ML models they were developing. P07 mentioned several key critical thinking questions that AI/ML practitioners do not ask themselves today, such as `\textit{Is this RAI value applicable to our product?}', `\textit{how does this value translate in diverse use cases?}' `\textit{should this value be enabled through the product?}'

% 1.1: Defining values in complex hi-stakes domain
%%The issue of deeper engagement becomes particularly important in high-stakes situation, such as healthcare where certain conditions have unequal impact on particular demographics. \fixme{P12} experienced this complexity while overseeing development of a ML models focused on health recommendations, 
%%\newline

%%\begin{quote}
%%    ``\textit{So a lot of models are geared towards ensuring that we have we are predictive about a health event and that almost always depends on different clinical conditions. For example, certain ethnic group can have more proclivity to certain health risks. So, if your model is learning correctly, it should make positive outcomes for this group more than the other groups. Now, if you blindly apply RAI values it might seem that the model is biased against this group when in reality these group of people are just more likely to have this condition, which is a correct conclusion not a biased one.}''
%%\end{quote}

%%Such deeper analysis requires hand-on practice and training on the field and formal in RAI education. However, both are hard to achieve today owing to RAI being a relatively nascent field.


%% 1.3 Contextualizing Eliciting values for multiple stakeholders. 
%%\item[Internal conflict of UX Practitioners] 
%%Challenges around critically engaging with RAI values was also much more complicated for certain roles. User-facing roles such as user experience researchers/designers, or program/product managers had the responsibility to understand, internalize, and embody end-user values in addition to their own values. We found that practitioners in these roles had to invest more effort to tease out their own values from that of the end-users. One such example was P04, a user experience researcher working on interfacing a large language model for natural conversations with users. A key RAI value they were interested in bringing forward to their team was explainability of the model. In process, they found it challenging to tease out and contextualize what explainability meant to themselves as a UX researcher as opposed to end-users that their model was serving. P04 described how through explainability, they were interested in getting better insights into the specific issues within the model's behavior (i.e. interpretability \cite{doran2017}). However, end-users were interested in translating opaque behaviors of the ML model (i.e. comprehensibility \cite{doran2017}). A UX Researcher is, however, expected to be the voice of the user in the process. So, they have to constantly ensure that they represent the values they have elicited appropriately.
%%\newline

%%Layers: Certain roles like UX and PM are responsible for advocating RAI values at different layers. For example, UX researchers advocate for explainability of ML models (which needs to materialize differently) than explainability for end-users (P04). Also end-user vs. intermediate users (P16).

% challenge-2: Values set at top
%%\item[Organizational Structures and Prioritizing RAI Values] 
%%Different organizational structures afforded prioritizing specific RAI values, and to varying degrees of support when providing resources.

%%While top-down RAI processes also facilitated RAI value elicitation from AI/ML practitioners, we discovered a few challenges in this approach. First, in comparison to bottom-up value elicitation practices, top-down practices experienced limited flexibility in open-discovery and discussion around diverse RAI values that mattered to their ML models or their projects. Most practitioners who shared values in top-down structures were restricted to engage with specific pre-determined RAI values that the company had deemed to be the `\textit{key}' RAI values. Moreover, the decision-making around what RAI values were consider key for the company happened at the management level. P06, an engineer at a large tech company working in conversational analysis models described his experience with eliciting RAI values, 
%%\newline
%%\begin{quote}
%%``\textit{To be honest, I imagine lots of the conversations around the sort of ethics of the various probes we were taking on happened above my pay grade. By the time the project landed on my desk to actually work. the ethics of it must have been cleared or kind of been punted to a later stage, given that it was kind of in the research space. }''
%%\end{quote}

%% 2.1: No time to elicit values in top-down structures.

%%Another challenge for practitioners invoking RAI values in top-down structures was the limited portion of the total time and the priority that was dedicated to open-ended RAI exploration, especially in the early stages of the product development. \fixme{P12}, an research scientist working in large-scale technology company shared how the focus in industry was first on improving the computational values of the model. Once computational values reached a certain benchmark, then practitioners like him were incentivized to spend their time on RAI values focused on ethics (e.g., fairness) or social justice (e.g., equity). Consequently several RAI practitioners skipped RAI value exploration and instead directly focused on implementing predetermined RAI values by the company just before the deployment. A few participants even mentioned implementing specific RAI values in the subsequent deployments only once they received initial reports of specific bias or social issues.

%% Speaker 2: [00:18:15] So in industry, everything is a little more fast paced because the goal is to achieve certain accuracy or certain quality metrics. So you can try different tricks which are not so unlike, which are not generalizable. Like you clean the data in a specific way and it gives you a boost because you are fine tuning your techniques for that particular application or that particular dataset. So the dynamics are more to do. Quick things, try out and feel frustrated. And in academia the focus is slightly different. The focus is on novelty of the algorithm and coming up with a little more general technique, which is applicable in a broader sense. Mm hmm. What ends up happening with that is sometimes the algorithms become super complex that they don't get implemented in the industry because the industry focuses on, like, simplifying things for one particular application. So. That is the main, I think, tension between the two. Okay. And. [00:19:21][66.4]


% 2.2: prefer not to share values  Approvals, additional work:  Don’t share values instead of additional approvals [D10], additional work.

% So uphoalding privacy value, as I mentioned, it was a challenge for us. So they have data setting. They want to-- that they have only certain tools which we can access to. For example, they are using a tool called BI in Incorta*. It's for-- and then that in Incorta*, they have their own set of machine learning libraries which we need to use. Now, if let's say I want to use some package or something else which is needed. Which I want to use for my model. It's a long chain process that we need to send it for approval. And, you know, then they would see, okay, if it's worth it or if they can incorporate it. If not, then we can--we have to simply look for an alternative




% RAI Compliance over other RAI concerns. 
% Speaker 2: [00:13:40] I say in the in the complaint, in the profit cases, usually top down, like it's like, you know, some some executive, some like high level executives, like why are all of our competitors doing this? And we're not doing this. And then then you find out, well, our audit our audit function doesn't have or like our compliance and audit function don't have any standard. So like when you when you send them something like this, they're like, what is this? Everything else you send this like there's like we know how we know how to measure it. Whereas this, like you need to create some sort of internal benchmark that we can then audit again or that we can then like approve again.  [00:14:21][40.3]


==> drafts/5-1overview.tex <==
% \section{Findings}
% Our overall findings are divided into four sections. The first section provides an introduction to the overall RAI structures that are being setup in the industry. The second section dives deeper into these structures by exploring how AI/ML practitioners share and co-produce RAI values in their teams. The third section explores different disagreements and conflicts that arise in the collaboration process to generate consensus on RAI values. The last section looks at some of the alignment strategies that the AI/ML practitioners undertake to solve the disagreements.

% \subsection{Current RAI Structures in the Industry}

% In our study we found that RAI conversations happened in three different ways. 

% \bheading{Bottom-up}
% One way RAI values have become part of workplace practices is through innovation happening at the lower echelons of the organization. In our interviews, eight participants from four different companies experienced or initiated bottom-up practices that engaged with RAI values.


% One of the enablers for such bottom-up innovation was individuals' sense of responsibility towards producing AI/ML models that did not lead to any harm in the society. These individuals encouraged and convinced their teams to engage with RAI values in order to minimize the potential harm of their ML models or AI products. These individuals mobilized their teams to seek out RAI resources available within and outside their organization. On occasion, when such resources were not available, individuals established their own RAI value levers that could be leveraged by other members within the organization as well. For instance, P08, a program manager, in a large-scale technology company shared how she started a semi-structured workshop to encourage and support their team members to come together and share RAI values, find commonly grounded definitions, contextualize RAI values to their products, and prioritize those values to implement in their projects. P08 described her experience of starting one bottom-up structure

% \begin{quote}
%     ``\textit{The initiative started with keen interest in socially responsible [AI] research and ultimately products. But we cater to projects that are very self-determined, very bottom up which aligned to sort of, you know, aligned values and priorities within the organization \dots These are what I call responsible innovation vigilantes around the company. I have also started that way but have grown into something more than that. But you'll see this at the product level or at the research team level, where somebody will speak up and say, `Hey, I want to be responsible for these values and make this my job and find solutions'. So you start to see individuals in different pockets of the company popping up to do that stuff.}''
% \end{quote}

% \bheading{Top-down}



% % RAI Compliance over other RAI concerns. 
% % Speaker 2: [00:13:40] I say in the in the complaint, in the profit cases, usually top down, like it's like, you know, some some executive, some like high level executives, like why are all of our competitors doing this? And we're not doing this. And then then you find out, well, our audit our audit function doesn't have or like our compliance and audit function don't have any standard. So like when you when you send them something like this, they're like, what is this? Everything else you send this like there's like we know how we know how to measure it. Whereas this, like you need to create some sort of internal benchmark that we can then audit again or that we can then like approve again.  [00:14:21][40.3]



==> drafts/5-2_copy.tex <==
\section{Findings}
Our overall findings are divided into four sections. The first section provides an introduction into the overall RAI structures that are being set up in the industry. The second section dives deeper into these structures by exploring how AI/ML practitioners share and co-produce RAI values in their teams. The third section explores different disagreements and conflicts that arise in the collaboration process to generate consensus on RAI values. The last section looks at several alignment strategies that AI/ML practitioners undertake to solve the disagreements.

\subsection{Practitioners' RAI Value Elicitation}

\bheading{Bottom-up Approaches}
One of the key ways in which RAI conversations  developed in industry was through RAI value sharing in lower echelons of organizations. AI/ML practitioners at this level shared their RAI values within their own teams in a bottom-up manner. In our interviews, eight participants from four different companies experienced or initiated bottom-up practices that engaged with RAI values.

One of the enablers for such bottom-up innovation was individuals' sense of responsibility towards producing AI/ML models that did not lead to any harm in society. Several social factors bolstered this feeling experienced by practitioners in their work and personal settings. For instance, \fixme{P22}, a user experience researcher working on \fixme{..} shared how her first hand experience of end-users on the ground formed her opinion about which RAI factors she could prioritize. Similarly, a few other practitioners paid close attention to `\textit{social climate}' (e.g., LGBTQ month, hate speech incidents) to elicit particular RAI values. 


Such individuals encouraged and convinced their teams to engage with RAI values in order to minimize the potential harm of their ML models or AI products. They mobilized their teams to seek out RAI resources available within and outside their organization. On occasion, when such resources were not available, individuals established their own RAI value levers that could be leveraged by other members within the organization as well. For instance, \fixme{P08}, a program manager, in a large-scale technology company shared how they leveraged scenario-based narratives and adversarial role plays in a semi-structured workshop. The activities encouraged and supported team members to come together and share RAI values, find commonly grounded definitions, contextualize RAI values to their products, and prioritize those values to implement in their projects. P08 described their experience of starting one bottom-up structure,

\begin{quote}
    ``\textit{The initiative started with keen interest in socially responsible [AI] research and ultimately products. But we cater to projects that are very self-determined, very bottom-up that aligned with our values and priorities within the organization \dots These are what I call responsible innovation vigilantes around the company. I have also started that way but have grown into something more than that. You'll see this at the product level or at the research team level, where somebody will speak up and say, `Hey, I want to be responsible for these RAI values and make this my job and find solutions'. So you start to see individuals in different pockets of the company popping up to do RAIstuff.}''
\end{quote}


Other value levers used by practitioners included conducting literature review of specific RAI values and understanding cutting edge methods, definition, and guidelines around them. To bring-in complementary RAI values into the team, several practitioners also deployed unconventional value levers. One example included \fixme{P18}, a data scientist working in a startup to host a panel in an attempt to capture complementary perspectives around AI explainability from different community roles like NGO and government to develop better explainable models. In a similar example, \fixme{P05}, a technical manager working on a reinforcement learning model in the context of healthcare for low resource in India,  facilitated field visits within the end-user communities to better understand what equitable model meant to them. 


% Speaker 2: [00:32:33] every panel, almost every panel had an intentional mix of factors represented. Mm hmm. So just like you said, somebody from an NGO, somebody from government, somebody in private industry, somebody in higher ed. Mm hmm. I would say that the most challenging. Group to include dovetailing on our. Well, we were talking about a moment ago, if that community representative.  [00:33:03][29.7]

RAI facilitators to encourage value sharing by AI/ML practitioners include
Sharing RAI values also enabled practitioners to disc

\bheading{Top-down Approaches}
Other opportunities of RAI value elicitation were facilitated by more concrete structures that were recognized, established, or integrated into the standardized workflows of the practitioners' teams to a varying degree. Consequently, these structures have allowed companies to establish checkpoints, pushing practitioners to think about RAI values around their products at individual and team level. We found a total of \fixme{12} individuals from 5 different companies who either implemented the RAI practices or facilitated them. P19, policy director of an RAI consultation agency described how such established structures enabled companies' to be more compliant.


% P19: So I think there's two things that can get you executive buy in. One is compliance. We're going to be sued or we were or this is a requirement under an upcoming law that we don't fulfill. And then the second thing is. A lack like putting up a barrier to profit. So, like, you know, our. We have for it. Like we have four major competitors. All of them have a system. We don't have an ad system because we don't have a responsible program that can judge its performance.
Teams that are asked to go and integrate RAI values (P10, P13). Or teams where RAI orgs are asked to go and serve
% P07: But they're very much laid down as a top down communication from executives to employees. Mm hmm. Um, you know, they weren't developed that way, but it's sort of not positioned as the centerpiece of the repeating. The products that are being launched will adhere to the principles or must adhere to it. So that's like a top down approach to responsible innovation


% P10: Speaker 1: [00:05:44] They came to us. They had already thought about some harms that could occur. And they said, Hey, here's our list of harms. Here's some ideas, the things we're doing for responsible air, what should we be doing? That was phenomenal. They'd already done pre-work. And this is in the sort of the yellow phase. Other time the teams have come to us and say, Hey, we want to publish and they want to publish within like a month of now. And they are like, What do we need to do for RTI point? I'm just like, You haven't thought about this at all. This is going to take a month, much more longer than a month to get you in good shape. [00:06:11][27.3]

% Speaker 1: [00:07:04] We have a bunch of bunch of internal Web pages that point you in all different types of directions. We don't have a singular voice that we speak with. And so because of that, we have that hodgepodge of some teams come to us willingly. Some teams come to us because they've been told to. Sometimes we're told you need to go track down this team because they're all doing stuff and they might need your help. [00:07:25][20.7]







%P19: H.R. bias one just for easier simplicity, like just for simplicity, if you're trying to comply with the like, any requirements to be able to explain every time you get adverse action like why that would be much easier if you also had an explainability program, if you also had like the had done some sort of bias testing on it. And so by kind of packaging these things together as like one thing, like rather like the responsibility AI certification organizations are able to see how. The different pieces fit together and how it's easier to do all of them than to take them piecemeal.  [00:17:31][53.4]


% When practitioners want to influence the RAI direction
% P05: Right. Say, for example, the privacy, right? So there's a huge, you know, myth or what you call the differences between what we understand as a privacy within Google and what external parties or partners understand as the privacy. Say you write a simple mail saying that, okay, we want to get a sample of your data to see whether the data fits our need, right. And it should be de-identified and the PI data should not be there. But despite saying this, the understanding of what is privacy within Google and what is outside is different. Like probably, they'll just remove the patient name and phone number and you'll have a hospital doctor. Of course, with this information, you can definitely trace back, if someone is interested, trace it back to the patient, right. So we need to explicitly mention, this is what we mean by privacy, right. And we have to take care. So that's one way of enforcing, like in sort of, like, a statement of work, we clearly have to make a statement. So these are the privacies we are looking for



\bheading{Challenges in Sharing RAI Values}

% challenge-1: Superficial
Despite the keen interest to share and communicate RAI values with their teams, we saw several challenges that hindered practitioners' intent and actions. A key issue was practitioners' ability to engage with RAI values critically that went beyond superficial engagement. \fixme{P07} a policy advisor in a large technology company who regularly interacted with such RAI implementers described such superficial engagement process as `\textit{moralizing}', wherein practitioners did not know how to develop deeper interpretations and contextualization of the elicited values around models they were developing. 

% challenge-2: Values set at top
While top-down RAI processes also facilitated RAI value elicitation from AI/ML practitioners, the specific RAI values itself were fixed at a much higher level. For instance, 
Pay-grade: If the RAI strategies happen top-down, RAI values can be set at a very high level. Stakeholders directly involved in the model do not get to decide which values are important (e.g., 6 values set by big org) [D25] .

P06: Uh, nothing that I noticed to be honest. I imagine lots of the conversations around the sort of ethics of the various probes we were taking on happened. You know, above my pay grade, so to speak. By the time the project landed on my desk to actually work on me the ethics of it must have been cleared or kind of been punted to a later stage, given that it was kind of in the research space. 

% RAI Compliance over other RAI concerns. 
% Speaker 2: [00:13:40] I say in the in the complaint, in the profit cases, usually top down, like it's like, you know, some some executive, some like high level executives, like why are all of our competitors doing this? And we're not doing this. And then then you find out, well, our audit our audit function doesn't have or like our compliance and audit function don't have any standard. So like when you when you send them something like this, they're like, what is this? Everything else you send this like there's like we know how we know how to measure it. Whereas this, like you need to create some sort of internal benchmark that we can then audit again or that we can then like approve again.  [00:14:21][40.3]



==> drafts/5-2discourses.tex <==
\subsection{Discourse \& Deliberations in RAI Value Co-production}



\bheading{Value Prioritization}

% Deliberations can occur at any stage of the life-cycle. Few teams were proactive , started RAI deliberation early in the ML life-cycle stage. These followed bottom-up approach. 

% Brainstorming values
% Prioritization of values 
% Finalize the values
% Embed the values through activities

% In our experience, very few teams proactively reached out early in the stage. A few teams that realize during 





% 1.3 Challenge: Pigeon hole values
%A key challenge with such dark horse values is that teams are often confined to a very narrow perspectives. 

% P8: [00:40:14] So one team came and really congratulated themselves about how they were dealing with fairness. It came out through the discussion that really they were congratulating themselves on procedural fairness when they really also needed to be focused on distributive fairness in terms of performance of the algorithm and then just like data ingestion. So I don't know what you take from that, but that was like one like very salient thing that I was like, okay, it was like kind of a basic thing [00:40:43][29.2]

\bheading{Tensions \& Challenges within Deliberations}
While practitioners found different opportunities to engage in coproduction activities, we saw several challenges around organization structures, roles, and values themselves that hindered such practices. In this section, we go through these categories in detail.
% Different organizational structures afforded prioritizing specific RAI values, and to varying degrees of support when providing resources. While top-down RAI processes also facilitated RAI value elicitation from AI/ML practitioners, we discovered a few challenges in this approach.
\subsubsection{Organizational Structures Challenges}
% Rigidity in Open-discovery

% \begin{figure*}
% \centering
% \includegraphics[width=\linewidth]{images/grid.png}
% \caption{Caption}
% \label{strip1}
% \end{figure*}

% Another challenge for practitioners invoking RAI values in top-down structures was the limited portion of the total time and the priority that was dedicated to open-ended RAI exploration, especially in the early stages of the product development. \fixme{P12}, an research scientist working in large-scale technology company shared how the focus in industry was first on improving the computational values of the model. Once computational values reached a certain benchmark, then practitioners like him were incentivized to spend their time on RAI values focused on ethics (e.g., fairness) or social justice (e.g., equity). 


%% Speaker 2: [00:18:15] So in industry, everything is a little more fast paced because the goal is to achieve certain accuracy or certain quality metrics. So you can try different tricks which are not so unlike, which are not generalizable. Like you clean the data in a specific way and it gives you a boost because you are fine tuning your techniques for that particular application or that particular dataset. So the dynamics are more to do. Quick things, try out and feel frustrated. And in academia the focus is slightly different. The focus is on novelty of the algorithm and coming up with a little more general technique, which is applicable in a broader sense. Mm hmm. What ends up happening with that is sometimes the algorithms become super complex that they don't get implemented in the industry because the industry focuses on, like, simplifying things for one particular application. So. That is the main, I think, tension between the two. Okay. And. [00:19:21][66.4]


% 2.2: prefer not to share values  Approvals, additional work:  Don’t share values instead of additional approvals [D10], additional work.

% So uphoalding privacy value, as I mentioned, it was a challenge for us. So they have data setting. They want to-- that they have only certain tools which we can access to. For example, they are using a tool called BI in Incorta*. It's for-- and then that in Incorta*, they have their own set of machine learning libraries which we need to use. Now, if let's say I want to use some package or something else which is needed. Which I want to use for my model. It's a long chain process that we need to send it for approval. And, you know, then they would see, okay, if it's worth it or if they can incorporate it. If not, then we can--we have to simply look for an alternative




% RAI Compliance over other RAI concerns. 
% Speaker 2: [00:13:40] I say in the in the complaint, in the profit cases, usually top down, like it's like, you know, some some executive, some like high level executives, like why are all of our competitors doing this? And we're not doing this. And then then you find out, well, our audit our audit function doesn't have or like our compliance and audit function don't have any standard. So like when you when you send them something like this, they're like, what is this? Everything else you send this like there's like we know how we know how to measure it. Whereas this, like you need to create some sort of internal benchmark that we can then audit again or that we can then like approve again.  [00:14:21][40.3]







% 1.1 Company’s values
%%In addition to the practitioners' familiarity with particular RAI values, 


% 1.2 sed on the RAI values that were methodologically easier to implement. In our interviews, a few practitioners (\fixme{n=XX}) found their team members often negotiated for accuracy over interpretability as model benchmarks (e.g., P/E ratio) because it was easier and computationally cheaper to implement, compared to model debugging techniques (e.g., SHAP).  
% Dark horse values

\paragraph{Inefficiency and Repair}
In other instances, unanticipated developments in RAI deliberations resulted in navigating the company's non-standardized approvals, thereby significantly altering the project timeline. For example, P23, an ML engineer shared how when they received issues around fairness from other stakeholders, it meant ``\textit{substantial changes to the model from the ground-up, because most of the time, issues with fairness stem from the data}''. It meant revisiting the data and redoing data collection or further debugging to remove the issues. Moreover, new and untested RAI values (e.g., interpretability) required more time and effort from the practitioners during implementation. RAI facilitators are essential in easing the tension in such situations by engaging in back-and-forth conversations with the teams to reduce the effort, streamline the process, and help practitioners appreciate the eventual consequences of implementing the RAI values. 

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{images/RAItable.png}
\caption{Table showcasing different values levers along side different properties observed in the study}
\label{strip1}
\end{figure*}

\paragraph{Perceived Misuse of RAI Values}
Lastly, practitioners observed tensions between their efforts in co-producing and implementing RAI values and their organization's use of such efforts for the overall business. For instance, P15, research director of a large-scale technology company overseeing research in large language models, shared how he was actively supporting a few teams in his company to co-produce and embed explainability into their models. However, he also expressed his concern on how companies could misrepresent such embedded RAI values,

\begin{quote}
    ``\textit{I worry that explainable AI is largely an exercise in persuasion. `This is why you should trust our software' rather than `This is why our software is trustworthy'. And so and I'm not saying everybody who does explainable AI is doing that kind of propaganda work, but it's a risk. Why do we want our AI to be explainable? Well, we'd like people to accept it and use it \dots Explainability part is ethically complicated \dots even for explainability for the practitioners the company wants it to be explainable, transparent, reliable, all those things as a means to an end. And the end is `please like our model, please buy our software'}''
\end{quote}

We found two more practitioners who raised similar concerns with other RAI values, such as privacy and trust. They were concerned that making their product ``\textit{completely responsible}'' could enable companies to market their products as nearly perfect, leading to overtrust and over-reliance. 

\subsubsection{Inter-Personal Practitioner Challenges}
% Different value-interpretation
Several conflicts also emerged as different roles interpreted and contextualized RAI values differently during the value deliberations. One form of tension were \textit{within practitioners} when different practitioners defined RAI values (e.g., equity) and mapped them to RAI features and metric (e.g., skin tone) differently. \fixme{P18}, a senior data scientist leading an AI team in a non-profit institute, shared one such similar tension but among their team members working on the same project,

\begin{quote}
    ``\textit{Probably half of my colleagues do believe that there is a cultural, and historical set of RAI values that can be applied to all the products organization wide. Other half are vehemently opposed to that concept and say that [RAI] values are always model and project dependent. So if you are talking about our long-term goal to establish a set of RAI principles, whose perspectives should be considered?\dots This is an uneasy space that needs careful navigation.}''
\end{quote}

On other occasions, a few practitioners disrupted the planned RAI deliberations by bringing in \textit{dark-horse} RAI values. These values were not part of the initially shortlisted RAI values built on the team's conversation. Instead, they were brought out from the side and championed by a very vocal practitioner, often at the later stages, who felt deeply about it. Dark horse RAI values also became a part of the discussion when practitioners in the team uncovered last-moment issues (e.g., bias) that significantly impacted the model.


Another set of tensions also occurred between \textit{practitioners and end-users}. P22, an Analyst in a financial firm, described how ML practitioners perceived RAI values to be mutable and negotiable, allowing them to implement a particular RAI value in stages instead of all at once. Such a process allowed P22 (and \fixme{three} other participants who reported similar narratives) to build the required experience and embed the value in the ML model or AI product. However, end-users expected these embedded RAI values as absolute and non-negotiable and not on a ``\textit{sliding spectrum}'' because they are ``\textit{they are often the list of ignored rights}'', leading to practitioner-user RAI tensions. 

\subsubsection{RAI Value Implementation Challenges}
RAI values also occupied overlapping and contesting spaces because some values have been historically better supported to provide teams with resources to implement them. We refer to this as \textit{Internal Value Feasibility}. First, practitioners were constantly conflicted between prioritizing RAI values that could be easily measured quantitatively against a baseline as opposed to RAI values that were abstract and did not have a measurement baseline. An example observed in this category was the contrast between RAI values like interpretability, which had concrete implementation techniques and measurements (e.g., LIME) and non-maleficence, which did not have a clear implementation technique or measurements. Similarly, in our interviews, a few practitioners (\fixme{n=3}) found their team members often negotiated for accuracy over interpretability as model benchmarks (e.g., P/E ratio) because it was easier and computationally cheaper to implement, compared to model debugging techniques (e.g., SHAP). 


For example, P19 mentioned how benchmarks are important when making choices to implement one RAI value or the other:

% Speaker 2: [00:13:55] And then then you find out, well, our audit our audit function doesn't have or like our compliance and audit function don't have any standard. So like when you when you send them something like this, they're like, what is this? Everything else you send this like there's like we know how we know how to measure it. Whereas this, like you need to create some sort of internal benchmark that we can then audit again or that we can then like approve again. And so, so yeah, it, it can start top down in the profit case and then and then bottom up and like another case, but like either way and like compliance becomes like a huge, like the lawyers want to come in and, and it kind of gets their like in the interest of navigating the corporate bureaucracy, the the legal compliance concerns can become heightened above like other responsible agencies.  [00:14:52][56.2]

%2.2 conflict in implementing one value which is in conflict with other. 

Yet values might end up competing with each other during implementation stage, that affects feasibility of the final solution.  We refer to this as \textit{Cross-Value Feasibility}. Second, co-producing and subsequent implementation of RAI values created conflicts with other RAI values. For instance,  \fixme{P1}, an engineer working on classification models in VR environments shared how their decision to improve accuracy by excluding instances of objects with sensitive cultural meanings (e.g., objects with LGBTQ references) also had direct repercussions on the diversity and fairness of the model. Implementing RAI values also created \textit{cascading} dependencies on the inclusion of other RAI values. For instance, \fixme{P16}, a program manager working as an RAI facilitator for a big tech company, shared the issues team members experienced around cascading RAI values:

\begin{quote}
   ``\textit{One common issue I see is with teams that are deadline with model Fairness issues. Most often the solution for them is to improve their datasets or sometimes even collect new forms of demographic data to retrain their model and that opens up another rabbit hole around privacy that the team now has to navigate through and ensure that their data adhere to our privacy standards. In most cases, teams don't even realize they are creating a new issue while trying to solve their existing problem \dots they also come for guidance when they don't know what to do around this new issue that they have opened up. } ''
\end{quote}

Finally, feasibility was challenged at the boundaries of organizations as they prioritized them differently rendering some values as infeasible , referred to as "External Feasibility". The last set of tensions occurred when organization' business values were in tension 
%with the RAI values practitioners were co-producing. It was especially evident where companies were developing and maintaining AI/ML products 
with those of external clients. In such cases, the team's commitment to engage with RAI was at odds with clients' business priorities. P02, a technical program manager for a service company that developed ML models for clients in the energy sector, had a similar issue when their team was building a model for street light automation. After P02's team received the data and started developing the model, they pushed for the value of safety. However, it was at odds with the company's value of efficiency,

\begin{quote}
    ``\textit{We should prioritize model optimization in those areas where there are higher crime rates \dots we don't want blackouts, right? \dots Their argument was if that a very high crime rate, such areas will also have high rate of purposefully damaging the lighting infrastructure. Prioritizing service to such areas will only create high amounts of backlogs as people will just vandalize it again. \dots So they just have different priorities. After that, our team just stopped following it up as it went into the backlog. }''
\end{quote}

P02 gave up prioritizing RAI values altogether after their clients either deprioritized multiple attempts to make them RAI ready or took an extremely long time to approve the requests. 



==> drafts/5-3-.tex <==
\subsection{Representations of Value Levers in Co-production}

\subsection{Value Levers as Strategies to Reduce Tensions} % can be integrated with the prior section.

\bheading{Institutional Value Levers}

Several practitioners \fixme{(n=15)} found engaging with their team members and knowing their perspectives helped them translate their RAI values into concrete and functional methods that applied to specific situations. To this end, we found participants taking advantage of several value levers that allowed conversations and receiving feedback (see Fig.\ref{Roles}). 



\begin{figure*}
\centering
\includegraphics[width=\linewidth]{images/VLRoles.png}
\caption{Heat map grid showcasing different values levers along side different roles that use them}
\label{Roles}
\end{figure*}



% 3. Ambiguous spaces bring deeply held values together

% P-4: [00:46:13] And so I think like a lot of this, space is very ambiguous and bringing the only thing that saves us in ambiguous spaces, I think, are our deeply held values. Like because ambiguous spaces are just that they are empty voids where we are trying to make the next decision to put our foot into a cloud. Right. Like and the only way that we can do that is by feeling our way through with values and being a team with shared values.  [00:46:37][24.5]



% 1. Using value levers to ensure that the participants reach alignment early in the process. Daily meetings

%%Other value levers to create safe spaces for value alignment included creating dedicated time called ``\textit{micro-meetings}'' that lasted about 15 minutes to enable open-discussion among the team members. These meetings were used to create and share collaborative manuscripts, such as google docs and presentation slides that captures the key ideas and facilitated alignment discussion around the micro-meetings in the offline space.
% 2. Values levers, user stories to Influence and persuade users








%%\bheading{Creating Structures for Positive Disagreements - SEEMS LIKE A SOLUTION}
%%During RAI value coproduction, we saw user-facing practitioners create explicit opportunities for disagreements and healthy conflicts to improve the quality of their teams' deliberations. Disagreements in coproduction phase allowed practitioners like UX researchers and product managers to go broad, capture diverse perspectives and expert knowledge %that different roles accumulated around their model functionalities, but did not not get an opportunity to share them with others over the time. 
%%prioritization framework. In the starting phases of this framework, the UX researcher pushed team members to go broad and co-produce values by wearing other practitioner's hats and invoking their RAI values. This practice allowed them to bring forward interesting disagreements between different roles that were then resolved and prioritized to achieve a small set of RAI values. Other top-down RAI programs also facilitated similar structures, explicitly providing narratives that brought out disagreements, eg: 
%P08, shared their experience:

%%\begin{quote}
%%    ``\textit{Usually I will write something in the prompts that I think that the team absolutely needs to hear about but is controversial and opposing. But I'm putting it into the voice of this engineering team so that it is not coming from us. It is not us scrutinizing them. That promotes interpersonal negotiation that pushes individuals to really defend their values with appropriate reasoning.}''
%%\end{quote}

% We also saw conflicts that disrupted the coproduction processes

%%\bheading{Business priorities vs. RAI values}
% 4. business priorities are in tension with the RAI values. 
%%The last set of conflicts occurred when companies' business values were in tension with the RAI values practitioners were co-producing. It was especially evident where companies were developing and maintaining AI/ML products for external clients. In such cases, the team's commitment to engage with RAI was at odds with clients' business priorities. P02, a technical program manager for a service company that developed ML models for clients in the energy sector, had a similar issue when their team was building a model for street light automation. After P02's team received the data and started developing the model, they pushed for the value of safety. However, it was at odds with the company's value of efficiency,

%%\begin{quote}
%%    ``\textit{We should prioritize model optimization in those areas where there are higher crime rates \dots we don't want blackouts, right? \dots Their argument was if that a very high crime rate, such areas will also have high rate of purposefully damaging the lighting infrastructure. Prioritizing service to such areas will only create high amounts of backlogs as people will just vandalize it again. \dots So they just have different priorities. After that, our team just stopped following it up as it went into the backlog. }''
%%\end{quote}

%%P02 gave up prioritizing RAI values altogether after their clients either deprioritized multiple attempts to make them RAI ready or took an extremely long time to approve the requests. 
% 1. Business needs outweigh the RAI needs [C36]. Clients do not take RAI values seriously. For example designing an ML model to be friendly vs. being equitable (P04).

% cutting business costs, dogfooding that often are at crossroads with RAI [D36]

%%
%%Another point of tension was when companies prioritized beta testing of ML models or AI products with the internal teams without considering their RAI values. In our study, three large-scale companies conducted internal beta testing to improve the embedded performance values (e.g., performance against human workers) in the model. These tests overlooked the RAI values of the teams that they were beta-testing, leading to pushback. For example, a content strategy team consisting of P03, was chosen to work with machine translation team to beta test the ML model for translation. From the initial stages of collaboration, P03's team found the model lacked explainable features that explained how the model was translating the content and how it could use the content. P03's team found it difficult to trust the model's output and requested the ML team with questions such as, ``\textit{what content has been used to train the model?}'', ``\textit{how is the accuracy calculated?}'', ``\textit{why is accurate in particular instances?}''. Consequently, the team had mixed feelings about testing the model for a longer duration, which translated in significant resistance to test the model. The team often ended up redoing the model's work to ensure it's accuracy. \fixme{Similar resistance has also been seen among data workers who have been seen as practitioners who are at the periphery of the ML model development \cite{wang2022}.}

% P3: [00:34:06] t's interesting because what we've been asked for is what is what is your what is your least valuable content? Do you have any content you're publishing where you don't really care that much about the translations and that that's not actually very difficult because it demeans the work that we do is unimportant. Like we don't think anyone reads the help center in the first place. So it's fine if we cut costs and we use your help center to train our machine learning and that that communication makes us really hesitant to say, yeah, we'd love to help you out because we we don't.  [00:34:38][31.7]
% Stakeholders championing non-established RAI values get more resistance 



% superficial or unethical ways of using the RAI values to the serve the means to the end of the business.
%%Lastly, practitioners also observed tensions between their efforts in co-producing and implementing RAI values and companies' use of such efforts for the overall business. For instance, P15, research director of a large-scale technology company overseeing research in large language models, shared how he was actively supporting a few teams in his company to co-produce and embed explainability into their models. However, he also expressed his concern on how such embedded RAI values could be leveraged by the company,

%%\begin{quote}
%%    ``\textit{I worry that explainable AI is largely an exercise in persuasion. This is why you should trust our software rather than this is why our software is trustworthy. And so and I'm not saying everybody who does explainable AI is doing that kind of propaganda work, but it's a risk. Why do we want our AI to be explainable? Well, we'd like people to accept it and use it \dots Explainability part is ethically complicated \dots even for explainability for the practitioners the company wants it to be explainable, transparent, reliable, all those things as a means to an end. And the end is `please like our model, please buy our software'}''
%%\end{quote}

%%We found two more practitioners who raised similar concerns with other RAI values, such as privacy and trust. They were concerned that making their product `completely responsible' could enable companies to market their products as nearly perfect, leading to overtrust and realiace. 

% Speaker 2: [00:43:13]  [00:43:47][33.9]


%%\bheading{Work Agency vs. RAI values}
% 3. Personal role, agency are in conflict with RAI values.
% 3.1 Personal impact on product is compromised by RAI value deliberation process.
%%Second tension was between RAI value coproduction and implementation and the practitioner's impact on the ML model or the AI product. \fixme{P13}, an ML engineer and RAI advocate, shared how individuals in their teams ``\textit{wanted to have their impact felt}'' in the development of the deep learning model and saw discussions and work around RAI as a direct conflict to their time dedicated for their work. 
%3.2 When RAI value implementations (or required changes) impact project timelines
%%Individuals required reassurance that their participation in such deliberations did not impact their work. In other instances, unanticipated developments in RAI deliberations resulted in navigating the company's non-standardized approvals, thereby significantly altering the project timeline. For example, P23, an ML engineer shared how when they received issues around fairness from other stakeholders, it meant ``\textit{substantial changes to the model from the ground-up, because most of the time, issues with fairness stem from the data}''. It meant revisiting the data and redoing data collection or further debugging to remove the issues. Moreover, new and untested RAI values (e.g., interpretability) required more time and effort from the practitioners during implementation. RAI facilitators are essential in easing the tension in such situations by engaging in back-and-forth conversations with the teams to reduce the effort, streamline the process, and help practitioners appreciate the eventual consequences of implementing the RAI values. 



==> drafts/5-3copy.tex <==
\subsection{RAI Value Co-production}
Having understood different opportunities of RAI value elicitation in different companies at an individual level, we now outline how RAI values were co-produced and prioritized within the teams.

\subsubsection{Enablers of Co-production}
In our interviews, we found several motivating factors that created a conducive environment for co-production of RAI values. One of them was overcoming the challenge of contextualizing RAI values to their own projects and translating those values to concrete methods that applicable to the situation.

% 1. Easy to contextualize as a team
% Translating RAI values to actual methods and asking the right questions is a tough job to do on your own, co-producing values reduces the burden down the line

% 1.1 collective experiences
% P06: And then, you know, we were very deliberate about Representing these data points as best we can. Right. So this is a male of this ethnicity, of this age with this kind of voice, you know, between like whatever. So we were quite explicit in terms of Trying To represent on that Front and then Using various permutations of the data available to us along those axes to try and make that obviously. So to your initial question, it's sort of as a team decision, it is largely derived off experience in terms of what we can expect from the model given These kind of inputs and do our work to as best we can call up buckets along these often quite sensitive sort of.

% 2. RAI programs (top-down and bottom-up): Different internal RAI programs and policies enable bottom-up/top-down collaboration [E35].
%P20: So the process that we follow is usually because we have a certain set of guidelines, we usually brainstorm with the actual product team first with respect to these values. So we would, you know, we want the product to be efficient and robust. We want it to be fair, transparent, accessible, and we want to make sure the data is private. And to do that, we then have these like a lot of conversations with the product team about how we can do that for that feature


% 2.2 Integrating RAI programs require collaboration between product teams and RAI teams. PMs for RAI value co-production and RS for RAI implementation

% "P07: No, no. I think the most fruitful conversations are actually with product managers. Oh, because they, you know, they have a more holistic view of the development of research and products. So they are more able to. Help us understand how our decisions and how the things that we do fit into the workflows of the for development. Research scientists are great and they offer very valuable perspectives, but they're a little less. They're more specific and a little less high level. And depending on the impact that you want to have, it's typically more useful to be on the product manager side. But as individuals, we work with a lot of research scientists and suffering engineers who, you know, who give us feedback on what does and doesn't work and why it makes sense."

\subsubsection{Value Prioritization}
Not all values that were thought out and expressed by the practitioners ended being implemented by the team. Instead, RAI values were constantly negotiated, prioritized, and vetted before. We found several factors that went into such processes.

% 1. Value familiarity and standardization
% Familiar Values are prioritized in a serial manner. Familiar values like privacy and security are prioritized over transparency and explainability [c18]. Mostly because of confirmation bias.

% "P20: Exactly. And so. A lot of times, like you would--the ideal situation would be like, ""Ooh, I have, like, six principles. I want to make sure our product has or addresses all those six principles in the first go. That's usually not how it happens. It usually happens sequentially. So like first and foremost, people will look at data and privacy 'cause that's super important. Everyone knows about it. They already have done probably some work around it. And then after that, they're like, ""Okay, now let's look at fairness,"" and then they'll probably look at explainability. And then--so it's usually very sequential because also research and industry is very quick and the turnaround is like one or two months.
% "

% Dark horse values: Dark Horse value is prioritized sometimes. It is problematic because the RAI value hijacks and disrupts a planned co-production approach [c4].

% P8: [00:45:24] Like sometimes what'll happen is like they'll do some negotiation about it and you get to like a list of six or something and then someone will bring up some like dark horse value that wasn't mentioned before at all, but then suddenly very important to the conversation and what was what's really interesting to me about that. So for a group where you're talking to machine learning, core machine learning researchers, this happened in book. We got to the same set of values, as I mentioned before, and both groups in my group, it was dark horse value of sustainability where that didn't come out of the initial discussions. But then somebody was like, What about sustainability? And you know? And then that influenced the conversation and end up becoming one of the four.
\subsubsection{Value Collaboration}

==> drafts/5-3representations.tex <==
\subsection{Representations of Value Levers in Co-production}

\subsection{Value Levers as Strategies to Reduce Tensions} % can be integrated with the prior section.

\bheading{Institutional Value Levers}

Several practitioners \fixme{(n=15)} found engaging with their team members and knowing their perspectives helped them translate their RAI values into concrete and functional methods that applied to specific situations. To this end, we found participants taking advantage of several value levers that allowed conversations and receiving feedback (see Fig.\ref{Roles}). 

\paragraph{Engineers \& Model Cards} We found that engineers created succinct representations and simplified documentation to share model details with the RAI values. When shared, such documentation helped them inculcate values and receive feedback from other roles in the team. P23, a senior engineer at an AI startup looking into sustainability, shared the process:
    \begin{quote}
    % quote needs to be updated
    `\textit{Even we have introduced this concept of a model card, wherein if a model is developed, the model card has to be filled out. So what is a model card? A model card is a series of questions that captures the basic facts about a model at a model level at an individual model level. What did you use to build a model? What was the population that was used? What is the scoring population? It is like, having all of that in a centralized standard format? Goes a long way to roll it up because the product can be very complex as well, right? With multiple players and whatnot. But having that ground of information collected in this way benefits the leads or the product owners, right}'
    \end{quote}


% \begin{figure*}
% \centering
% \includegraphics[width=\linewidth]{images/VLRoles.png}
% \caption{Heat map grid showcasing different values levers along side different roles that use them}
% \label{Roles}
% \end{figure*}

\paragraph{UI/UX Practitioners \& Visual Tools} UI/UX designers, UX researchers, and analysts also used similar documentation tools to initiate discussions and receive feedback from other practitioners in the team. \fixme{P20}, a UX researcher, used presentation slides containing model features to facilitate brainstorming sessions and receive feedback from other roles. They also used FigJam containing key RAI values and user findings to initiate affinity diagramming, allowing the team to ``\textit{categorize the findings and map them to specific RAI values}''. Other RAI levers included designing and sharing info-graphics and regular RAI standups where practitioners took it upon themselves to be stewards of RAI principles for the team to give updates, receive feedback and learn about team's perspectives on specific RAI values.


The aforementioned user-facing roles, including program/product managers, also had the responsibility to understand, internalize, and embody end-user values in addition to their own values. We found that practitioners in these roles had to invest more effort to tease out their own values from that of the end-users. One example was P04, a user experience researcher working on interfacing a large language model for natural conversations with users. A key RAI value they were interested in bringing forward to their team was the \textit{explainability} of the model. In the process, they found it challenging to tease out and contextualize what explainability meant to themself as a UX researcher as opposed to the end-users that their model was serving. While P04 was interested in getting better insights into the model's behavior issues (i.e. interpretability \cite{doran2017}), end-users were interested in a simplified understanding of the model's opaque behavior (i.e. comprehensibility \cite{doran2017}). A UX Researcher is, however, expected to be the voice of the user in the process. Consequently, they had the constant burden to elicit both sets of values appropriately.  

\paragraph{Managers, RAI Leaders \& Certifications} 

\blue{RAI programs initiated within the organizations also created similar but formal structures for practitioners and their teams to facilitate coproduction. Example structures included designing and propagating standardized guidelines, such as guidebooks, around established RAI values, such as fairness and accountability, bringing in expert lecturers to share their experiences around coproduction, and enabling shared spaces for coproduction. Such shared spaces enabled product/program managers or equivalent roles provided a holistic view of the market fit of the product. UX researchers, and designers highlighted the user needs, and implications of lack of attention to the RAI values. We noticed that Research scientist, software engineer, data scientist, or equivalent roles provided specific details of the research and implementation. Together, these insights led to discussions about how RAI values could fit into different model development workflows. } 

Interestingly, we found independent agencies offering RAI programs as `\textit{Responsible AI certifications}'. These certifications target AI/ML start-ups and organizations in sectors, such as energy, mining, and human resources that often have a limited technology workforce. These external programs act as facilitators between the non-technology and technology workforce by enabling coproduction around RAI values to make them compliant with upcoming regulations. They did this by packaging different activities under the RAI certification program, such as getting buy-in for particular RAI values, leveraging trusted partners for running impact assessments, engaging key actors in value discovery and prioritization, and implementing appropriate RAI methods. For example, \fixme{P19} described effort of facilitating RAI value conversations within their client teams as a key part of the certification process:

    \begin{quote}
    ``\textit{It is important to have everybody on board for those [RAI] value conversations. So we try really hard to have all the different teams like internal or external audit, legal, business, data and AI team come together, brainstorm, discuss different [RAI] issues in specific contexts and shortlist [the RAI values], even if we just get a little bit of their time \dots everyone needs to be brought in early because we conduct a lot of activities likes audit analysis, bias testing\dots it saves time, addresses several concerns, and establish streamlined [RAI] processes. \dots For simplicity, we just package all of the different activities we do under RAI certification.}''
    \end{quote}

% 3. Ambiguous spaces bring deeply held values together

% P-4: [00:46:13] And so I think like a lot of this, space is very ambiguous and bringing the only thing that saves us in ambiguous spaces, I think, are our deeply held values. Like because ambiguous spaces are just that they are empty voids where we are trying to make the next decision to put our foot into a cloud. Right. Like and the only way that we can do that is by feeling our way through with values and being a team with shared values.  [00:46:37][24.5]


\subsubsection{Bottom-up Frameworks}
During RAI value coproduction, we saw user-facing practitioners create explicit opportunities for disagreements and healthy conflicts to improve the quality of their teams' deliberations. Disagreements in coproduction phase allowed practitioners like UX researchers and product managers to go broad, capture diverse perspectives and expert knowledge %that different roles accumulated around their model functionalities, but did not not get an opportunity to share them with others over the time. 
For example, \fixme{P04}, a UX researcher, created bottom-up adversarial prioritization framework. In the starting phases of this framework, the UX researcher pushed team members to go broad and co-produce values by wearing other practitioner's hats and invoking their RAI values. This practice allowed them to bring forward interesting disagreements between different roles that were then resolved and prioritized to achieve a small set of RAI values. Other top-down RAI programs also facilitated similar structures, explicitly providing narratives that brought out disagreements, eg: 
%P08, shared their experience:

\begin{quote}
    ``\textit{Usually I will write something in the prompts that I think that the team absolutely needs to hear about but is controversial and opposing. But I'm putting it into the voice of this engineering team so that it is not coming from us. It is not us scrutinizing them. That promotes interpersonal negotiation that pushes individuals to really defend their values with appropriate reasoning.}''
\end{quote}
\fixme{According to P19, having such RAI system in place early also allows companies to judge it’s ML models benchmarks when compared to their competition.}

% 1. Using value levers to ensure that the participants reach alignment early in the process. Daily meetings

\subsubsection{Safe Spaces for Disagreements}
Despite several tensions in the coproduction of RAI values, we also found different RAI value levers that focused on reducing them and improving value alignment. One key alignment strategy was to create structures and activities that aligned the team's RAI values pretty early in the process. One such activity that we saw in both practitioner's and RAI programs was providing ``\textit{safe spaces}'' to encourage open discussions among individuals to empathize with other members. \fixme{P09} shared,

\begin{quote}
    ``\textit{One alignment strategy was open discussion with the safe space, where team members could fail, be called out and to learn from each other as we were developing values. So say someone finds the value of democratization really important, they are made to articulate what they mean by it.\dots. It is easy if there are different buckets in which they can categorize and explain because then people can easily surface all the different ways they think and prioritize values and that helps with alignment}''
\end{quote}

%%Other value levers to create safe spaces for value alignment included creating dedicated time called ``\textit{micro-meetings}'' that lasted about 15 minutes to enable open-discussion among the team members. These meetings were used to create and share collaborative manuscripts, such as google docs and presentation slides that captures the key ideas and facilitated alignment discussion around the micro-meetings in the offline space.
% 2. Values levers, user stories to Influence and persuade users

\subsubsection{User Stories/Scenarios to Build Empathy}
Another set of value levers used especially by the roles facing end-users was user stories and scenarios to influence and persuade users to change their value priorities and align with rest of the team. These levers were also used by the roles to converge on key values after engaging in healthy conflicts within the divergence phase. For example, \fixme{P04}, exposed different pain points and key journeys of users by ``\textit{highlighting clip of a user that is really, really amazing story that is either very painful or poignant}''. Interestingly, P04 was aware how such value levers had to be evoked carefully,

\begin{quote}
    \textit{``If that story is not representative, I'm manipulating the system. If it is representative, I'm influencing the system...So I will not operate on the side of manipulation. So I like to be very squarely on the side of influence. And I do like regular checks for myself to make sure that I am operating on influence, not manipulation, in terms of the stories that I am allowing people to amplify.''}
\end{quote}

% 3. Office hours or one-on-one consultation to iron out the differences.
\subsubsection{Office Hours to Diffuse Tensions}
The last alignment-focused value levers were \textit{RAI office hours}, which were part of top-down RAI programs (\fixme{n=2}). These office hours were available for elicitaion, production, and tension-resolution.
%%also accessible, in addition to RAI value elicitation, to the teams who were experiencing tensions around RAI values and perceived roadblocks in implementing them. 
A typical office hour was 30 minutes in which practitioners engaged with a relevant expert and an experienced facilitator. One key way experts solved the tensions in these sessions was by providing concrete case-study examples. For example, P21, an RAI office hour facilitator, shared an example when his Office hours were used. The practitioners were at odds with each other in implementing explainability and transparency features. During the office hours, P21 responded by sharing a few edge case scenarios like that of pregnant women who had just lost a child and might need a form of explainability that allows them to change the model's behavior. 

%%\bheading{Creating Structures for Positive Disagreements - SEEMS LIKE A SOLUTION}
%%During RAI value coproduction, we saw user-facing practitioners create explicit opportunities for disagreements and healthy conflicts to improve the quality of their teams' deliberations. Disagreements in coproduction phase allowed practitioners like UX researchers and product managers to go broad, capture diverse perspectives and expert knowledge %that different roles accumulated around their model functionalities, but did not not get an opportunity to share them with others over the time. 
%%prioritization framework. In the starting phases of this framework, the UX researcher pushed team members to go broad and co-produce values by wearing other practitioner's hats and invoking their RAI values. This practice allowed them to bring forward interesting disagreements between different roles that were then resolved and prioritized to achieve a small set of RAI values. Other top-down RAI programs also facilitated similar structures, explicitly providing narratives that brought out disagreements, eg: 
%P08, shared their experience:

%%\begin{quote}
%%    ``\textit{Usually I will write something in the prompts that I think that the team absolutely needs to hear about but is controversial and opposing. But I'm putting it into the voice of this engineering team so that it is not coming from us. It is not us scrutinizing them. That promotes interpersonal negotiation that pushes individuals to really defend their values with appropriate reasoning.}''
%%\end{quote}

% We also saw conflicts that disrupted the coproduction processes

%%\bheading{Business priorities vs. RAI values}
% 4. business priorities are in tension with the RAI values. 
%%The last set of conflicts occurred when companies' business values were in tension with the RAI values practitioners were co-producing. It was especially evident where companies were developing and maintaining AI/ML products for external clients. In such cases, the team's commitment to engage with RAI was at odds with clients' business priorities. P02, a technical program manager for a service company that developed ML models for clients in the energy sector, had a similar issue when their team was building a model for street light automation. After P02's team received the data and started developing the model, they pushed for the value of safety. However, it was at odds with the company's value of efficiency,

%%\begin{quote}
%%    ``\textit{We should prioritize model optimization in those areas where there are higher crime rates \dots we don't want blackouts, right? \dots Their argument was if that a very high crime rate, such areas will also have high rate of purposefully damaging the lighting infrastructure. Prioritizing service to such areas will only create high amounts of backlogs as people will just vandalize it again. \dots So they just have different priorities. After that, our team just stopped following it up as it went into the backlog. }''
%%\end{quote}

%%P02 gave up prioritizing RAI values altogether after their clients either deprioritized multiple attempts to make them RAI ready or took an extremely long time to approve the requests. 
% 1. Business needs outweigh the RAI needs [C36]. Clients do not take RAI values seriously. For example designing an ML model to be friendly vs. being equitable (P04).

% cutting business costs, dogfooding that often are at crossroads with RAI [D36]

%%
%%Another point of tension was when companies prioritized beta testing of ML models or AI products with the internal teams without considering their RAI values. In our study, three large-scale companies conducted internal beta testing to improve the embedded performance values (e.g., performance against human workers) in the model. These tests overlooked the RAI values of the teams that they were beta-testing, leading to pushback. For example, a content strategy team consisting of P03, was chosen to work with machine translation team to beta test the ML model for translation. From the initial stages of collaboration, P03's team found the model lacked explainable features that explained how the model was translating the content and how it could use the content. P03's team found it difficult to trust the model's output and requested the ML team with questions such as, ``\textit{what content has been used to train the model?}'', ``\textit{how is the accuracy calculated?}'', ``\textit{why is accurate in particular instances?}''. Consequently, the team had mixed feelings about testing the model for a longer duration, which translated in significant resistance to test the model. The team often ended up redoing the model's work to ensure it's accuracy. \fixme{Similar resistance has also been seen among data workers who have been seen as practitioners who are at the periphery of the ML model development \cite{wang2022}.}

% P3: [00:34:06] t's interesting because what we've been asked for is what is what is your what is your least valuable content? Do you have any content you're publishing where you don't really care that much about the translations and that that's not actually very difficult because it demeans the work that we do is unimportant. Like we don't think anyone reads the help center in the first place. So it's fine if we cut costs and we use your help center to train our machine learning and that that communication makes us really hesitant to say, yeah, we'd love to help you out because we we don't.  [00:34:38][31.7]
% Stakeholders championing non-established RAI values get more resistance 



% superficial or unethical ways of using the RAI values to the serve the means to the end of the business.
%%Lastly, practitioners also observed tensions between their efforts in co-producing and implementing RAI values and companies' use of such efforts for the overall business. For instance, P15, research director of a large-scale technology company overseeing research in large language models, shared how he was actively supporting a few teams in his company to co-produce and embed explainability into their models. However, he also expressed his concern on how such embedded RAI values could be leveraged by the company,

%%\begin{quote}
%%    ``\textit{I worry that explainable AI is largely an exercise in persuasion. This is why you should trust our software rather than this is why our software is trustworthy. And so and I'm not saying everybody who does explainable AI is doing that kind of propaganda work, but it's a risk. Why do we want our AI to be explainable? Well, we'd like people to accept it and use it \dots Explainability part is ethically complicated \dots even for explainability for the practitioners the company wants it to be explainable, transparent, reliable, all those things as a means to an end. And the end is `please like our model, please buy our software'}''
%%\end{quote}

%%We found two more practitioners who raised similar concerns with other RAI values, such as privacy and trust. They were concerned that making their product `completely responsible' could enable companies to market their products as nearly perfect, leading to overtrust and realiace. 

% Speaker 2: [00:43:13]  [00:43:47][33.9]


%%\bheading{Work Agency vs. RAI values}
% 3. Personal role, agency are in conflict with RAI values.
% 3.1 Personal impact on product is compromised by RAI value deliberation process.
%%Second tension was between RAI value coproduction and implementation and the practitioner's impact on the ML model or the AI product. \fixme{P13}, an ML engineer and RAI advocate, shared how individuals in their teams ``\textit{wanted to have their impact felt}'' in the development of the deep learning model and saw discussions and work around RAI as a direct conflict to their time dedicated for their work. 
%3.2 When RAI value implementations (or required changes) impact project timelines
%%Individuals required reassurance that their participation in such deliberations did not impact their work. In other instances, unanticipated developments in RAI deliberations resulted in navigating the company's non-standardized approvals, thereby significantly altering the project timeline. For example, P23, an ML engineer shared how when they received issues around fairness from other stakeholders, it meant ``\textit{substantial changes to the model from the ground-up, because most of the time, issues with fairness stem from the data}''. It meant revisiting the data and redoing data collection or further debugging to remove the issues. Moreover, new and untested RAI values (e.g., interpretability) required more time and effort from the practitioners during implementation. RAI facilitators are essential in easing the tension in such situations by engaging in back-and-forth conversations with the teams to reduce the effort, streamline the process, and help practitioners appreciate the eventual consequences of implementing the RAI values. 


